Deep equilibrium models as estimators for continuous latent variables

Principal Component Analysis (PCA) and its exponential family extensions have three components: observations, latents and parameters of a linear transformation. We consider a generalised setting where the canonical parameters of the exponential family are a nonlinear transformation of the latents. We show explicit relationships between particular neural network architectures and the corresponding statistical models. We find that deep equilibrium models -- a recently introduced class of implicit neural networks -- solve maximum a-posteriori (MAP) estimates for the latents and parameters of the transformation. Our analysis provides a systematic way to relate activation functions, dropout, and layer structure, to statistical assumptions about the observations, thus providing foundational principles for unsupervised DEQs. For hierarchical latents, individual neurons can be interpreted as nodes in a deep graphical model. Our DEQ feature maps are end-to-end differentiable, enabling fine-tuning for downstream tasks.

==> figures/algorithm.tex <==
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\begin{algorithm}
\caption{\texttt{PED.forward($Y, \theta, C$)} }\label{alg:map}
\begin{algorithmic}
\Require Data point $Y \in \mathbb{R}^{d_0}$. Parameters $\theta$ containing weights $W^{(l)} \in \mathbb{R}^{d_{l-1} \times d_{l}}$ and biases $b^{(l)} \in \mathbb{R}^{d_l}$ for each $1 \leq l \leq L-1$, number of iterations $C$. 
\Ensure A local MAP estimate $({z^{(1)}}^\ast, \ldots, {z^{(L)}}^\ast)$ of $p \Big( z^{(1)}, \ldots, z^{(L)} \mid Y, \theta \Big)$.
\State $z^{(l)}(0) \gets (0, \ldots, 0) \in \mathbb{R}^{d^{(l)}}$ for each $1 \leq l \leq L$.
\State $c \gets 1$
\While{$c \leq C$ \textbf{or} $\big| z^{(l)}(c) - z^{(l)}(c-1) \big| \leq \text{TOL}$ for $1 \leq l \leq N$}
\State $z^{(0)}(c) \gets Y$
\If{$c$ is odd}
\State $z^{(l)}(c) \gets \text{Update}\big(z^{(l-1)}(c), z^{(l+1)}(c-1) \big)$ for each $1 \leq l \leq L$
\Else
\State $z^{(l)}(c) \gets \text{Update}\big(z^{(l-1)}(c-1), z^{(l+1)}(c) \big)$ for each $L > l \geq 1$
\EndIf
\State $c = c + 1$
\EndWhile
\State ${z^{(l)}}^\ast = z^{(l)}(C)$ for each $1 \leq l \leq L$
\end{algorithmic}
\end{algorithm}


==> figures/bayesnet_orthogonal.tex <==
\begin{figure*}[!ht]
    \centering
        \centering
            \begin{tikzpicture}
            % Define nodes
              \node[obs]                                (y) {$Y_s$};
              \node[latent, above=of y, xshift=0.5cm]   (Q) {$\mathsf{Q}$};
                \node[latent, above=of y, xshift=-0.5cm]   (b) {$B$};
              \node[latent, right=of y]                  (z) {$Z_s$};
                \node[latent, above=of z]               (K) {$\mathsf{K}$};
                
              % Connect the nodes
              \edge {z,Q,b} {y} ; %
              \edge {K} {z};
            
              % Plates
              \plate[inner sep=0.35cm] {yz} {(z)(y)} {$s=1,\ldots,N$} ;
            \end{tikzpicture}
            \begin{align*}
            Y_s &\sim \expfam(H_s), \quad H_s = \mathsf{Q} Z_s + B \\
            Z_s &\sim \mathcal{N}(0, \lambda^{-1}\mathsf{K}) \\
            \mathsf{Q} &\sim \mathcal{U}\big((\mathbb{O}(d,l) \big) \\
            \mathsf{K} &\sim \mathcal{W}, \\
            B &\sim \mathcal{N}(0, \gamma^{-1} \mathsf{I} )
        \end{align*}   
    \caption{The graphical model for linearly parameterised exponential family PCA using orthonormal bases $\mathsf{Q}$ and conditionally Gaussian latents $Z_s$ each with covariance matrix $\mathsf{K}$. Here $\mathcal{U}\big(\mathbb{O}(d,l) \big)$ denotes the probability distribution corresponding with the normalised Haar measure supported on $\mathbb{O}(d,l)$, i.e. a type of uniform distribution over semi-orthogonal matrices. $\mathcal{W}$ is a Wishart distribution over the space of (symmetric) positive definite matrices.}
    \label{fig:bayes_nets_orthogonal}
\end{figure*}

==> figures/bayesnet_relu.tex <==
\begin{figure}
    \centering
        \begin{tikzpicture}
          % Define nodes
          \node[obs]                                (y) {$Y_s$};
          \node[latent, above=of y, xshift=0.5cm]   (w) {$W$};
            \node[latent, above=of y, xshift=-0.5cm]   (b) {$b$};
          \node[latent, right=of y]                  (z) {$Z_s$};
        \node[latent, below=of y]                   (eps) {$\epsilon_s$};
          % Connect the nodes
          \edge {z,w,b,eps} {y} ; %
        
          % Plates
          \plate[inner sep=0.35cm] {yz} {(z)(y)(eps)} {$s=1,\ldots,N$} ;
        \end{tikzpicture} \\
    \begin{align*}
        Y_s &\sim \text{ExpFam}\big( \text{ReLU}(H_s) \big), \quad H_s = W Z_s + b \\
        Z_s &\sim \mathcal{N}(0, \lambda^{-1}I) \\
        W, b &\sim \mathcal{N}(0, \gamma^{-1} I ) \\
        \epsilon &\sim \mathcal{N}(0, \tau^2 I)
    \end{align*}   
            
    \caption{When the result of the linear transformation $WZ_s +b$ is mapped through the $\text{ReLU}$ before being passed as canonical parameters of an exponential family, MAP estimation becomes more involved; the first order derivative characterisation~\eqref{eq:deriv_eq_0} of the differentiable and strictly convex optimum in the non-ReLU case is lost due to the non-differentiability and non-convexity introduced by the ReLU. However, if an auxillary latent variable $\epsilon_s$ is introduced and marginalised out, the non-differentiable point of the ReLU is smoothed out. This marginalised MAP can be found using the EM algorithm, and uniqueness of the minimum can be guaranteed using a contraction assumption. When the limit of the variance $\tau^2$ of $\epsilon_s$ is taken to zero, the M-step is once again characterised by a first order derivative condition analagous to~\eqref{eq:deriv_eq_0}. Furthermore, only one iteration of EM is required, which can be solved using a DEQ.}
    \label{fig:bayes_nets_relu}
\end{figure}
